Combinatorial synthesis of cation-disordered manganese tin nitride MnSnN$_2$ thin films with magnetic and semiconducting properties

Magnetic semiconductors may soon improve the energy efficiency of computers, but materials exhibiting these dual properties remain underexplored. Here, we report the computational prediction and realization of a new magnetic and semiconducting material, MnSnN$_2$, via combinatorial sputtering of thin films. Grazing incidence wide angle X-ray scattering and laboratory X-ray diffraction studies show a wide composition tolerance for this wurtzite-like MnSnN$_2$, ranging from $20\% <$ Mn/(Mn+Sn) $< 65$\% with cation disorder across this composition space. Magnetic susceptibility measurements reveal a low-temperature transition ($T^{\mathrm{*}} \approx 10$ K) for MnSnN$_2$ and strong antiferromagnetic correlations, although the ordering below this transition may be complex. This finding contrasts with bulk MnSiN$_2$ and MnGeN$_2$, which exhibited antiferromagnetic ordering above 400 K in previous studies. Spectroscopic ellipsometry identifies an optical absorption onset of 1 eV for the experimentally-synthesized phase exhibiting cation disorder, consistent with the computationally-predicted 1.2 eV bandgap for the cation-ordered structure. Electronic conductivity measurements confirm the semiconducting nature of this new phase by showing increasing conductivity with increasing temperature. This work adds to the set of known semiconductors that are paramagnetic at room temperature and will help guide future work targeted at controlling the structure and properties of semiconducting materials that exhibit magnetic behavior.

==> Mn-Sn-N thin film synthesis paper (Version 8518)/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
